An Instrumental Value for Data Production and its Application to Data Pricing

How much value does a dataset or a data production process have to an agent who wishes to use the data to assist decision-making? This is a fundamental question towards understanding the value of data as well as further pricing of data. This paper develops an approach for capturing the instrumental value of data production processes, which takes two key factors into account: (a) the context of the agent's decision-making problem; (b) prior data or information the agent already possesses. We ''micro-found'' our valuation concepts by showing how they connect to classic notions of information design and signals in information economics. When instantiated in the domain of Bayesian linear regression, our value naturally corresponds to information gain. Based on our designed data value, we then study a basic monopoly pricing setting with a buyer looking to purchase from a seller some labeled data of a certain feature direction in order to improve a Bayesian regression model. We show that when the seller has the ability to fully customize any data request, she can extract the first-best revenue (i.e., full surplus) from any population of buyers, i.e., achieving first-degree price discrimination. If the seller can only sell data that are derived from an existing data pool, this limits her ability to customize, and achieving first-best revenue becomes generally impossible. However, we design a mechanism that achieves seller revenue at most $\log (\kappa)$ less than the first-best revenue, where $\kappa$ is the condition number associated with the data matrix. A corollary of this result is that the seller can extract the first-best revenue in the multi-armed bandits special case.

==> sections/back-ups.tex <==
SECTION 2 BACKUPS

We start by discussing a few nuances about quantifying the value of data, particularly, its  connection and distinction to the similar problem on the \emph{value of information}, which is much more well-understood in the literature of information economics \cite{bergemann2018design,frankel2019quantifying}. Clearly, data and information are related. At a high level, information can be viewed as the knowledge extracted from data, through common sense inference classically or through machine learning nowadays. Hence agents purchase data in the market aiming at obtaining some information. Data carries (partial) information, captured by the data generation process and information has both intrinsic value and instrumental value. We will give a way to value the information associated with certain data in the next sections. As for signals, unlike data which has a fixed format determined by the generation process, signals, as well as experiments and signaling schemes, are arbitrarily designed, interacting between sellers and buyers in the data market. Let's consider the following example to visualize these concepts. 
\begin{example}[Large language model training]\label{example:google}
Google hopes to train its large model, Gemini, to automatically price its advertising products, called Ad-Gemini. Therefore, it needs to purchase trading data from some trading companies. Google informed Company A about its goal, and Company A ultimately provided Google with nearly five years of private stock trading datasets that were most relevant to Google's objective. In the end, the transaction occurred, and Google provided Company A with a fee.
\end{example}
In \Cref{example:google}, what is contained in the private stock trading datasets of Company A, beneficial to the training of Ad-Gemini, is information while these private stock trading datasets are data. Besides, the goal informed by Google to Company A which may be different from its original goal, of automatically pricing its advertising products, is the signal in this transaction. 

{Then, we tell the difference between intrinsic value and instrumental value of data. Intrinsic value refers to the inherent worth of something, independent of any external factors or purposes. It is the value that something possesses in and of itself. However, instrumental value, on the other hand, refers to the usefulness of something in achieving a specific goal or purpose. This value is relative and depends on the utility of an object or action in realizing particular objectives. In essence, instrumental value is derived from the functionality of an item or behavior in relation to achieving other goals. In \Cref{example:google}, the datasets have intrinsic value as companies can use them to train arbitrary models while they have instrumental value when considering a specific model like Ad-Gemini. Intrinsic value is an inherent attribute while instrumental value depends on circumstances. If Google already uses these datasets to train Gemini, it's useless to leverage them to train Ad-Gemini, showing something with high intrinsic value may have little or even no instrumental value. In the data market, agents purchase data for specific purposes and care about the associated instrumental value contained in the data which is beneficial to certain goals. Therefore, in the following paper, we will focus on the instrumental value of data and how to price data and design mechanisms.
}

 With a more precise function $f_{\beta}(\cdot)$, the buyer can finally achieve his ultimate goal of estimating expected value in the direction of $x$, i.e. the conditional expectation function $f_\beta(x)$. At the same time, $f_\beta(x)$ is the estimator with the least mean square error (MSE) for estimating associated $y$.  , whereas assuming the buyer gives a \emph{feature} $\hat x$ as the signal, pretending to aim for corresponding \emph{response} $\hat y$. With the help of revelation principle~\citep{gibbard1973manipulation,holmstrom1978incentives,myerson1979incentive}, when we consider a mechanism design problem, there must exist an optimal mechanism where we can constrain the signal $\hat x$ in the feature space. Therefore, we adopt such restriction from now on without weakening our results. Recall that in \Cref{example:google}, the goal is to train Ad-Gemini, i.e. the conditional expectation function $f_\beta(x)$ where $x$ represents a task of pricing automatically but not an output $y$ with exogenous uncertainty. 


 {We use the following \Cref{fig:sec2} to depict the process. Notably, the information cared about by the buyer is the response $y$ then the true model $f_\beta(x)$, while not the tuple $(x,y)$,
since feature direction $x$ is supplied by the buyer. } 
Intuitively, we can regard $x$ as certain \emph{context} that the buyer cares about, and he aims to purchase some new data to enhance his knowledge of the statistical model's prediction along this direction. This is motivated by many practices where a learner collects responses to refine model estimation along a particular direction (e.g., a certain population of insureds or financial products from a certain category), and services such as  CrowdAI and Scale AI provide these responses ~\citep{CrowdAI, ScaleAI}.

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{sections/sec2.jpg}
    \caption{Information structure between the seller and the buyer. The buyer with type $x$ owns prior distribution $q$ over the parameter $\beta$ first. He reports $\hat x$ to the seller, receiving a dataset $\cD[\hat x]$ and being charged $t(\hat x)$. Then, he is able to obtain an updated posterior distribution over $\beta$ called $p$.}
    \label{fig:sec2}
\end{figure}


==> sections/info_gain.tex <==
 
  % \hf{For all the following contents in this section, I suggest we either remove them, or state them as lemmas to prove Theorem \ref{lem:infogain}. We should make it clear that Theorem \ref{lem:infogain} is the ONLY main result of this section.  
  
  
  % I think it is not important to emphasize information gain here, since more attractive to the readers is a concrete valuation function that they can work with. This is why I think Theorem \ref{lem:infogain} is perhaps the most important message of this section. Information gain is just an intermedia step employed to prove this theorem.  } 
  
  % Having justified the choice of information gain, we now proceed with deriving our main results under the proposed valuation function.





 

%  \begin{example}[Contextual Bandits with Linear Payoffs]\label{example:cbandits}
%     For contextual bandits with linear payoff functions~\citep{chu2011contextual}, it's assumed that the payoff related to context $x$ is $\langle x,\beta\rangle+\epsilon$. If an agent hopes to learn accurate payoff in the direction of $x$, he can purchase a dataset $\cD[\hat x]$ containing previous experimental data of this system. Utilizing the prior in his mind, he can shape a posterior and entropy is a natural measure of how well he understands the system under context $x$.
% \end{example}


%  We are now ready to show under such a scenario, information gain is a valid instrumental value of data. \hf{I suggest removing the following theorem. It is not surprising at all. Also, simply saying it is a "valid" value is not a strong statement as there are tons of valid ones, why this one is particularly interesting? I think Theorem \ref{lem:infogain}  is more interesting, since it shows that IG is the value associated with entropy. Since entropy is widely used, so we should also use IG. }  We assume $V(x,\cD[\hat x])$ is the information gain (c.f. \Cref{defn:info_gain}) when a buyer equipped with $x$ purchases $\cD[\hat x]$, then it is exactly the expected value of information in some decision-making problem, as defined in Definition~\ref{defn:val-info-cost-uncertainty}. 
% \begin{theorem}
%     \label{prop:ig-ex-ante-val-info}
%     There is a decision-making problem such that {the information gain} $\IG$ is the ex-ante value of data,  that is
%     \begin{equation*}
%         \textstyle
%         \IG(x, \cD[\hat{x}])=\EE_{\cD[\hat{x}] \sim g_q}[ \val(x, \cD[\hat{x}]; q) ] ,
%     \end{equation*}
%     where $q$ is the buyer's prior belief over $\beta$ and, with a slight abuse of notation, $\EE_{\cD[\hat{x}] \sim g_q}[\cdot]$ is the expectation taken over the buyer's belief about the purchased data $\cD[\hat{x}]$ under the prior $q$.
% \end{theorem}
% In other words, $\IG$ is exactly the expected value of $\cD[\hat{x}]$ to the buyer when he makes the purchase. The fact that $\IG$ is the buyer's ex-ante value of data is crucial, as it is impossible for the buyer to ascertain exactly the data's value to him prior to observing $\cD[\hat{x}]$ and updating his belief. {It justifies the choice of information gain and we list its detailed concept and closed form under Bayesian linear regression which provides some convenience for optimal mechanism design in \Cref{sec:optimal,sec:subopt}.}




% Before introducing information gain {formally}, we begin by recalling the definition of differential entropy, which generalizes the notion of information entropy from the discrete setting~\citep{shannon1948mathematical} to continuous random variables and measures the buyer's uncertainty.



% To reflect the fact that the data sold is affected by the buyer's own reported features, we let $\hat{x}$ denote the buyer's reported feature and $\cD[\hat{x}]$ the data the seller sends to the buyer. The buyer, having observed $\cD[\hat{x}]$, formulates a posterior belief over $\EE[y ( x)]$ according to Equation~\eqref{eq:posterior-update}, and we let the entropy over the posterior be $h(f_p(x))$, {where $p$ represents the posterior distribution over $\beta$}.

% With the prior and the posterior defined, we {give a formal introduction to information gain} in Bayesian regression.
% \begin{definition}[Information Gain]
%     \label{defn:info_gain}
%     For a buyer type $x$, the information gain from $\cD[\hat{x}]$ is
%     \begin{equation}
%         \label{eq:def-val-ig}
%         \IG(x, \cD[\hat{x}]) := h(f_q(x)) - h(f_p(x)),
%     \end{equation}
%     where $h(f_q(x))$ and $h(f_p(x))$ are the entropy of his prior and posterior distributions over $\EE[y (x)]$ {and $p$ depends on both $q$ and $\cD[\hat x]$}. 
%     % \hf{I think $h(y | x, \cD[\hat{x}])$ is a confusing notation when comparing with $h(y|x)$ since $h(y|x)$ is the distribution of $y$ given feature $x$, under some fixed prior $g$ over $\beta$. Technically, $h(y | x, \cD[\hat{x}])$ should denote  the distribution of $y$ given feature $x, \cD(\hat{x}$, which does not make sense here. Instead, it should be  the distribution of $y$ (still)given feature $x$ but $g$ is updated with data $\cD(\hat{x}$  --- am I correct? }
% \end{definition}





==> sections/intro-hf.tex <==
We hope this newly developed valuation function could serve as an alternative to Shapley value, particularly for usage in producing additional data to supplement certain decision making. 

Ours is more statistical whereas Shapley value is more computational. We require much less retraining, but depends on a useful cost function. 

Our value allows arbitrary data production process, whereas Shapley value is only defined for a data records. 

==> sections/mechanism.tex <==
\section{Optimal Pricing of Data Production using Canonical Valuations} 
% {\color{red}Sorry but a kind reminder. The DDL is 3pm CT on May 22nd, not AOE. }
In this section, we use the developed closed-form characterization for canonical valuations of DPPs in Section \ref{BLR} to study a natural optimal pricing problem for selling DPPs. While the choice of valuation functions generally may be domain-dependant, the goal of this section is to showcase a natural economic application of the newly developed   valuation functions of DPPs. We study how to sell data production processes (DPPs) to  a machine learner (henceforth, the \emph{buyer}). 

We consider the following standard mechanism design framework, albeit being instantiated in our DPP pricing setup with fundamentally different utility functions and allocation rules. Specifically, the buyer would like to estimate $y = \langle x, \beta \rangle$. The   decision context $x$ is buyer's private information, also conventionally referred to as the buyer \emph{type}, which is  unknown to the seller.  Unlike Bayesian mechanism design, we study \emph{prior-free} mechanism design which is known to be notoriously more challenging but much more practical due to free of assumption on seller's prior knowledge and on how buyer type is generated \cite{goldberg2001competitive,devanur2009limited}. The $\beta$ here is the to-be-estimated parameter by the buyer. For simplicity, we assume the buyer initially has no knowledge about the model parameter $\beta$; formally, buyer's initial belief $q = \cN(0,\Sigma_0)$ about $\beta$ is a standard Gaussian.\footnote{Our results can be generalized to general Gaussian prior (same for every buyer), but with more complex notations.} The buyer would like to buy data from the seller to refine his Bayesian posterior belief about $\beta$. 
Throughout this section, we assume seller's data production has no costs, though it is an interesting future direction to integrate cost of production. The remainder of this section presents our design of  optimal or approximately optimal mechanism, depending on how much power the seller as in customizing DPPs. 



 
 

In reference to the model displayed in \Cref{BLR}, the buyer is equipped with some {fixed} type vector $x$ in favor of related data-generating process and sends $\hat x$ to the seller, {akin to settings of mechanism design literature~\citep{myerson1979incentive,bull2007hard,borgers2015introduction}}. {$x$ and $\hat x$ might be different as the buyer pretends to ask for data corresponding to the direction of $\hat x$ in order to reduce the payment. }In the perfect customization case, the seller can directly, and potentially repeatedly, observe the response which corresponds to $\hat{x}$, namely $\hat y=\langle \hat x, \beta\rangle+\epsilon$, where $\epsilon\sim\cN(0,\sigma(\hat x)^2)$. For simplicity, we assume that the seller receives
$n$ measurements of $\hat{y}$, jointly independent when conditioned on $\hat{x}$ and $\beta$. {The size of the dataset, i.e. $n$, might depend on the cost of generating data and the budget constraints faced by the buyer which is exogenous and independent of our mechanism design. When $n$ is unknown, the seller will employ the following proposed mechanism in \Cref{algo:opt} concurrently with her personal cost function to derive the optimal $n$. We refer readers interested in further information on the cost function to \citet{herzog2010theory}. For the convenience of understanding, we assume $n$ is fixed from now on.}
% When the seller is $n$ is unknown, the seller will employ the following mechanism in conjunction with her personal cost function to derive the optimal 
% $n$. We refer readers interested in further information on the cost function to \citet{herzog2010theory}. 
In order to increase revenue, the seller may inject into the responses some artificial noise denoted by $\epsilon'$, where 
$\epsilon'\sim \cN(0,\delta(\hat x)^2)$. {The idea behind these artificial noises is that the seller hopes they can help distinguish buyers with a better willingness to pay. By injecting noise, it might punish buyers who misreport their own types and motivate a truthful mechanism. Then, the seller can utilize price discrimination to obtain higher expected revenue.} She then charges the buyer 
$t(\hat x)$, which may depend on 
$n$, {the number of data point in the dataset}. The exact timing line is provided in \Cref{fig:perfect}.




\subsection{The Power of Perfect Data Customization: Achieving the First Best}\label{sec:optimal}
% We first consider the following information flow which represents customization. Considering the model in \Cref{BLR}, the buyer has private type $x$ and reports $\hat x$ to the seller. The seller can help the buyer to gain customized data $\hat y=\langle \hat x, \beta\rangle+\epsilon$ where $\epsilon\sim\cN(0,\sigma(\hat x)^2)$. For simplicity, we assume the quantity of data is known and denoted by $n$. With unknown $n$, the seller will use the mechanism below and her own cost function to derive optimal $n$. Readers can learn more about cost function in \citet{herzog2010theory}. Since the seller hopes to achieve price discrimination, she would like to add some man-made noise $\epsilon'$. We assume that $\epsilon'\sim \cN(0,\delta(\hat x)^2)$. Then, the seller charges the buyer $t(\hat x)$ which contains $n$ implicitly.

% With the definition of $\IG(\cdot,\cdot)$ in \Cref{eq:def-val-ig}, we have the following lemma about the value of data. We assume that the prior distribution is $\cN(0,I_d)$\footnote{We don't use the characteristic that $\beta$ is finite-dimensional and it can be extended to reproducing kernel Hilbert space directly.} W.L.O.G. If $\Var(\beta_q)$ is not full-rank, it means that some directions are deterministic and we can simply wipe off them. For general priori $\cN(\beta_0,\Sigma_0)$, we can subtract every $y$ by $x^T\beta_0$ to reduce to the situation of $\cN(0,\Sigma_0)$. Then, we can replace $(x,\beta)$ by $(\sqrt{\Sigma_0}x,(\sqrt{\Sigma_0})^{-1}\beta)$ and it reduces to our assumption.

We begin with the case where the seller can customize her data perfectly. {Recall that we use ``customize'' to represent the seller will distribute different data after observing different reports of the buyer's type. ``Perfect'' here means that the seller can generate data after observing the report like in \Cref{fig:perfect} while we will use ``limited'' to represent the situation in which the seller generates data before receiving reports. We note that customization scenario often occurs between pharmaceutical companies and hospitals. Pharmaceutical companies hope that hospitals can help them evaluate the effectiveness of newly developed drugs. Therefore, pharmaceutical companies will pay for experiments conducted in hospitals. Although hospitals may not have the capability to produce drugs, they can provide observational data on the efficacy of drugs for pharmaceutical companies. We first adopt the following example to illustrate scenarios of perfect data customization. 
\begin{example}[Drug efficacy assessment]\label{example:drug}
    Pfizer has developed a new drug for the treatment of lung cancer and is seeking to conduct drug testing at Hospital B. Hospital B provided Pfizer with the following two options. 
    \begin{itemize}
        \item Hospital B directly conducts experiments on patients using the drug and returns clinical outcomes to Pfizer.
        \item Hospital B provides Pfizer with the results of previous lung cancer patients who have used other drugs.
    \end{itemize}
    Both options are beneficial for Pfizer to assess the effectiveness of the new drug and present different mechanism design problems for the study protocols.
\end{example}
In \Cref{example:drug}, the first option that the hospital uses drugs provided by Pfizer on patients directly is a kind of scenario of perfect data customization in the real world. In abstract terms, no matter what feature vector the buyer is interested in, the seller has the capability to generate precisely the data that the buyer desires.
}

In reference to the model displayed in \Cref{BLR}, the buyer is equipped with some {fixed} type vector $x$ in favor of related data-generating process and sends $\hat x$ to the seller, {akin to settings of mechanism design literature~\citep{myerson1979incentive,bull2007hard,borgers2015introduction}}. {$x$ and $\hat x$ might be different as the buyer pretends to ask for data corresponding to the direction of $\hat x$ in order to reduce the payment. }In the perfect customization case, the seller can directly, and potentially repeatedly, observe the response which corresponds to $\hat{x}$, namely $\hat y=\langle \hat x, \beta\rangle+\epsilon$, where $\epsilon\sim\cN(0,\sigma(\hat x)^2)$. For simplicity, we assume that the seller receives
$n$ measurements of $\hat{y}$, jointly independent when conditioned on $\hat{x}$ and $\beta$. {The size of the dataset, i.e. $n$, might depend on the cost of generating data and the budget constraints faced by the buyer which is exogenous and independent of our mechanism design. When $n$ is unknown, the seller will employ the following proposed mechanism in \Cref{algo:opt} concurrently with her personal cost function to derive the optimal $n$. We refer readers interested in further information on the cost function to \citet{herzog2010theory}. For the convenience of understanding, we assume $n$ is fixed from now on.}
% When the seller is $n$ is unknown, the seller will employ the following mechanism in conjunction with her personal cost function to derive the optimal 
% $n$. We refer readers interested in further information on the cost function to \citet{herzog2010theory}. 
In order to increase revenue, the seller may inject into the responses some artificial noise denoted by $\epsilon'$, where 
$\epsilon'\sim \cN(0,\delta(\hat x)^2)$. {The idea behind these artificial noises is that the seller hopes they can help distinguish buyers with a better willingness to pay. By injecting noise, it might punish buyers who misreport their own types and motivate a truthful mechanism. Then, they can utilize price discrimination to obtain higher expected revenue.} The seller then charges the buyer 
$t(\hat x)$, which may depend on 
$n$, {the number of data point in the dataset}. The exact timing line is provided in \Cref{fig:perfect}.

\begin{figure}[!htbp]
    \centering
    \includegraphics[width=\textwidth]{sections/perfect.jpg}
    \caption{Timing line for perfect data customization. {The first step is to announce the mechanism to be used. Then, the buyer who is equipped with type $x$ gives a report $\hat x$ to the seller. The seller will base on $\hat x$ to produce a dataset we call $\cD[\hat x]$ and give it to the buyer. Finally, the buyer will give the seller a preset fee $t(\hat x)$.}}
    \label{fig:perfect}
\end{figure}

We assume without loss of generality {there is a common knowledge} that the prior distribution {over $\beta$} is 
$\cN(0,I_d)$\footnote{We do not use the fact that 
$\beta$ is finite-dimensional and our results can be directly extended to reproducing kernel Hilbert space.}{, which is standard in information economy literature~\citep{frankel2019quantifying,hartline2010bayesian,maschler2020game}.} If 
$\Var(\beta_q)$, {the variance matrix of the prior parameter,}
is not full-rank, this implies that certain directions are deterministic and can be disregarded. For a general priori 
$\cN(\beta_q,\Sigma_0)$, we can subtract every 
$y$ by 
$x^T\beta_q$ to simplify the situation to 
$\cN(0,\Sigma_0)$. Subsequently, we can replace 
$(x,\beta)$ by 
$(\sqrt{\Sigma_0}x,(\sqrt{\Sigma_0})^{-1}\beta)$ and it will reduce to our initial assumption.

Concerning the definition of $\IG(\cdot;\cdot,\cdot)$ in \Cref{eq:value-linear-dpp}, we can establish a lemma exhibiting the
concrete instrumental value of data in detail.
\begin{lemma}\label{lem:concrete_value}
    If the seller gives the buyer $n$ data points, it holds that the instrumental value of data
for the buyer is
\[
\IG(x, \widehat{x}):=\IG( \cD[\widehat{x}];\cN(0,I_d),x)=\frac{1}{2} \log \left(x^T x\right)-\frac{1}{2} \log \left(x^T\left(I+\frac{n \widehat{x} \widehat{x}^T}{\sigma(\widehat{x})^2+\delta(\widehat{x})^2}\right)^{-1} x\right).
\]
\end{lemma}

% With revelation principle \citep{gibbard1973manipulation,holmstrom1978incentives,myerson1979incentive}, we only consider the incentive-compatibility (IC) mechanism. Since the buyer is assumed rational, the mechanism should satisfy individual rationality (IR) constraints. Therefore, we formally state the following constraints that the mechanism should obey.
By revelation principle \citep{gibbard1973manipulation,holmstrom1978incentives,myerson1979incentive}, {we know that any social choice function implemented by an arbitrary mechanism can be implemented by an incentive-compatible-direct-mechanism with the same equilibrium outcome.} Therefore, we focus on mechanisms that satisfy incentive-compatibility (IC) constraint and {at least one optimal mechanism belongs to this subclass. In the context of our model, incentive-compatibility constraint means that the buyer has the motivation to report his own private type truthfully considering the allocation rule $\cD[\cdot]$ and payment rule $t(\cdot)$.} To ensure the buyer is motivated to purchase data, we further impose individual rationality (IR) constraints. {It means that a rational buyer only participates in a transaction when his expected revenue is no less than zero. }Formally, the IC and IR constraints for a mechanism $(\cD[\cdot], t(\cdot))$ are
\begin{align*}
    \label{eq:defn_ir}
    &\textrm{IR}  &\IG(x, x) &\geq t(x)\textrm{ for all }x,\\
    % \label{eq:defn_ic}
    &\textrm{IC}  &\IG(x, x) - t({x}) &\geq \IG(x, \hat x) - t(\hat x)\textrm{ for all }x, \hat{x} .
\end{align*}
{In other words, IC constraint means that truthful reporting is a dominant strategy for the buyer and he has no incentive to report a wrong type as there are no benefits by doing so. IR constraint gives the buyer a reason to join the market and motivates the transaction as his expected utility is non-negative.}

We further make an assumption on the data-generating model. {We assume the variance is scaled to the norm of the feature as follows.}
\begin{assumption}\label{assumption:scale}
The noise's variance scales with the length of $x$, i.e. $\sigma(x)=\sigma(\frac{x}{\|x\|})\|x\|.$
\end{assumption}

% Assumption \ref{assumption:scale} is a quite normal assumption in physics literature and biomedicine literature \citep{linnet1990estimation,kumar1994proportional,bland1996measurement} as the measurement error is often proportional to the quantitative of the variable. Also, we constrain the additive noise $\epsilon'$ also have a proportional variance that 
% \[
% \delta(x)=\delta(\frac{x}{\|x\|})\|x\|,
% \]which may reduce the seller's revenue. However, we will show as follows that such a family of mechanisms can already achieve the first-best revenue so the mechanism we propose is indeed the optimal mechanism.


Assumption \ref{assumption:scale} is commonplace in the literature of physics and biomedicine \citep{linnet1990estimation,kumar1994proportional,bland1996measurement,wang2006proportional}, as the measurement error is frequently proportional to the ``size'' of the variable being measured and here ``size'' is quantified by $\| \cdot \|$. Similarly, we stipulate that the additional noise 
$\epsilon'$ also has a proportional variance defined by $\delta(x)=\delta(\frac{x}{\|x\|})\|x\|$, which may decrease the revenue obtained by the seller. Nevertheless, we will demonstrate that this family of mechanisms is capable of achieving the first-best revenue and, by extension, optimality.

% With Assumption \ref{assumption:scale} in hand, it's obvious that we only can only consider the direction of type rather than the length. We can replace $x$ and $\hat x$ by $\frac{x}{\|x\|}$ and $\frac{\hat x}{\|\hat x\|}$ and it holds that
% \[
% \IG( x,\hat x)=\IG(\frac{x}{\| x\|},\frac{\hat x}{\|\hat x\|}).
% \]
% From now on, we only consider types belonging to $\{x:\|x\|=1\}$.
Given Assumption \ref{assumption:scale}, it is evident that we could solely consider the direction of the type, rather than its length. This can be achieved by substituting 
$x$ and $\hat x$
  with 
$\frac{x}{\|x\|}$ and $\frac{\hat x}{\|\hat x\|}$, respectively. We then have
\[
\IG( x,\hat x)=\IG(\frac{x}{\| x\|},\frac{\hat x}{\|\hat x\|}).
\]
We thus restrict our attention to types with a unit norm, i.e. 
$\cS^{d-1}=\{x:\|x\|=1\}$, {which is equivalent to considering a general space in $\RR^{d-1}$}. Inspired by the method in \citet{myerson1981optimal}, we have the following lemma when $x$ has multiple dimensions.
\begin{lemma}\label{lem:paymentgrad}
    For any payment rule satisfying the IC constraint, it holds that
\[
\nabla t(x)=\nabla_y \IG(x,y)\given_{y=x}.
\]
Therefore, it leads to the following form of payment rule that
\[
t(x)=\int_{x_0}^x \nabla_y \IG(x,y)\given_{y=x}\cdot dx+t(x_0)=\frac{1}{2}\log(\frac{\sigma(x)^2+\delta(x)^2+n}{\sigma(x)^2+\delta(x)^2})+C,
\]
and it's independent of the selection of $x_0$ and the path of integration.
\end{lemma}
{Compared with the well-known results of single-dimension in \citet{myerson1981optimal}, there are two main differences considering a multi-dimensional type. First of all, we need to generalize the derivation of a one-dimensional function to the gradient computation in the case of higher dimensions. Second, when calculating the payment rule $t(\cdot)$, the integral result is required to be independent of the initial starting point and the integral path we choose. In our situation, it means that no matter what $x_0$ and the path from it to the final $x$ we choose, the result of the integral should be the same. These conditions constrain the application scenarios of the extended method for multi-dimensional mechanism design as we only need monotonicity for the single-dimensional situation. Nevertheless, the proof will elaborate that our definition of instrumental value satisfies all these conditional endogenously, highlighting the importance of our framework of instrumental value and suggesting its broad range of applications.}

Therefore, for any $\delta(x)$, we have the corresponding optimization problem for optimal mechanism, that is
\begin{equation*}\label{optimization_problem}
      \max_{C,\delta(\cdot)} \EE_x t(x)=\EE_x [C+\frac{1}{2}\log(\frac{\sigma(x)^2+\delta(x)^2+n}{\sigma(x)^2+\delta(x)^2})]\ind({\rm IR\ holds}),
\end{equation*}
where $$\ind({\rm IR\ holds})=
  \ind(C+\frac{1}{2}\log(\frac{\sigma(x)^2+\delta(x)^2+n}{\sigma(x)^2+\delta(x)^2})+\frac{1}{2}\log(x^T(I+\frac{nxx^T}{\sigma(x)^2+\delta(x)^2})^{-1}x)\le 0).$$  

{Though information gain is a widely used metric, our analysis method can be extended to a wider family of instrumental values as long as keeping the concavity property as what $\log(\cdot)$ does. We add the following remark to show how to generalize our results.} 
\begin{remark}
The method can be easily extended to any $\IG(\cdot,\cdot)$ function following the form
\[
\IG(x,\hat x)=f(\frac{x^Tx}{x^T(I+\frac{\hat x\hat x^T}{(\sigma(\hat x)^2+\delta(\hat x)^2)/n})^{-1}x}),
\]
where $f(\cdot)$ is a concave function, and the results remain valid when $t(x)$ is of the form
\[
t(x)=C+f(\frac{\sigma(x)^2+\delta(x)^2+n}{\sigma(x)^2+\delta(x)^2}).
\]
\end{remark}

We now state our main result. {It shows that when the seller is embedded with the ability of perfect customization, she can obtain the first-best revenue and leave zero consumer surplus to the buyer. It reflects the price discrimination scenario in the data market and shows corresponding unfairness which is quite different than the situation in other markets.}
\begin{theorem}\label{thm:optimalmech}    {There exists a mechanism satisfying both IC and IR constraints} that for any $\sigma(\cdot)$ and prior distribution on the type $x$, the seller can achieve the first-best revenue and first-degree price discrimination, where the corresponding payment rule is 
    \[
    t(x)=\frac{1}{2}\log(\frac{\sigma(x)^2+n}{\sigma(x)^2}).
    \]
\end{theorem}

% We formalize \Cref{thm:optimalmech} in \Cref{algo:opt}. \Cref{algo:opt} shows in detail that when the seller has customization ability, there's no need for her to add additional noise besides endogenous ones. She can abstract the buyer's willingness to pay exactly since data in different directions may impair the buyer's valuation heavily. Therefore, for sellers with perfect data customization ability, it's achievable for them to achieve the first-best revenue with unfairness to buyers and society. 
We present an optimal mechanism constructed by \Cref{thm:optimalmech} in \Cref{algo:opt}. As demonstrated in \Cref{algo:opt}, when the seller can perfectly customize data, it is unnecessary for her to inject any additional noise. She can fully extract the buyer's willingness to pay since the value of data significantly degrades once the buyer alters the direction of the reported type. Consequently, for sellers with perfect data customization ability, it is feasible for them to achieve the first-best revenue at the expense of the buyers, {where the sellers seize all the surplus and none are left to the buyers}. Moreover, there is no deadweight loss (see \citet{hausman1981exact} for detailed concepts) since she is selling as much information as possible, without injecting any artificial noise, and the buyer has no further willingness to pay. The result stands in {distinct} contrast to the corresponding market forms for physical commodities.

% \begin{algorithm}[thbp]
% \renewcommand{\algorithmicrequire}{\textbf{Input:}}
% \renewcommand{\algorithmicensure}{\textbf{Output:}}
%     \begin{algorithmic}
%     \REQUIRE{buyer's report $\hat x$}
%     \STATE Set $\delta(\cdot)\equiv 0$ for the distribution of added noise $\cN(0,\delta(\cdot)^2)$
%     \STATE The seller generates $n$ data \hf{Is $n$ a design parameter, or a given fixed value in advance?} points following $\hat y_i=\hat x^T\beta+\epsilon_i+\epsilon'_i$ where $\epsilon'_i\overset{\text{i.i.d.}}{\sim}\cN(0,\delta(\hat x)^2)$
%     \ENSURE {
%          $\cD[\hat{x}] = \{(\hat x ,\hat y_i)\}_{i=1}^n$ and $t(\hat x)=\frac{1}{2}\log(\frac{\sigma(\hat x)^2+n}{\sigma(\hat x)^2})$
% }\label{algo:allocation}\label{algo:payment}
%     % Set $t(\hat{x}) = \IG(\hat x, \cD(\hat{x})) =\frac{1}{2}\log(\hat x^T\hat x)-\frac{1}{2}\log(\hat x^T(I+\sellX^Tb(\hat x)b(\hat x)^T\sellX)^{-1}\hat x)$\;
%     \caption{Pseudocode for the Optimal Mechanism}
%     \label{algo:opt}
%     \end{algorithmic}
% \end{algorithm}

% \begin{algorithm}[t]    
% 	\SetAlgoNoLine
% 	\KwIn{buyer's report $\hat x$}
% 	Set $\delta(\cdot)\equiv 0$ for the distribution of added noise $\cN(0,\delta(\cdot)^2)$\;
%  The seller generates $n$ data 
%  % \hf{Is $n$ a design parameter, or a given fixed value in advance?}
%  points following $\hat y_i=\hat x^T\beta+\epsilon_i+\epsilon'_i$ where $\epsilon'_i\overset{\text{i.i.d.}}{\sim}\cN(0,\delta(\hat x)^2)$\;
% 	\KwOut{$\cD[\hat{x}] = \{(\hat x ,\hat y_i)\}_{i=1}^n$ and $t(\hat x)=\frac{1}{2}\log(\frac{\sigma(\hat x)^2+n}{\sigma(\hat x)^2})$}\label{algo:allocation}\label{algo:payment}
% 	\caption{Pseudocode for the Optimal Mechanism}
%         \label{algo:opt}
% \end{algorithm}

\begin{algorithm}[htbp]
   \caption{Pseudocode for the Optimal Mechanism}
        \label{algo:opt}
\begin{algorithmic}
   \STATE {\bfseries Input:} buyer's report $\hat x$
   \STATE Set $\delta(\cdot)\equiv 0$ for the distribution of added noise $\cN(0,\delta(\cdot)^2)$;
   \STATE  The seller generates $n$ data 
 % \hf{Is $n$ a design parameter, or a given fixed value in advance?}
 points following $\hat y_i=\hat x^T\beta+\epsilon_i+\epsilon'_i$ where $\epsilon'_i\overset{\text{i.i.d.}}{\sim}\cN(0,\delta(\hat x)^2)$;
    \STATE {\bfseries Output:} $\cD[\hat{x}] = \{(\hat x ,\hat y_i)\}_{i=1}^n$ and $t(\hat x)=\frac{1}{2}\log(\frac{\sigma(\hat x)^2+n}{\sigma(\hat x)^2})$\label{algo:allocation}\label{algo:payment}
\end{algorithmic}
\end{algorithm}


% \Cref{thm:optimalmech} shows that when the seller has customization ability, she can achieve first price revenue and subtracts all buyer's surplus. At the same time, there's no deadweight loss (see \citet{hausman1981exact} for detailed concepts) that she sells as much information as she can and the buyer has no more willingness to pay. So, under this information flow, there is a market with unfairness that the buyer enjoys no surplus and it shows large differences with corresponding market forms for physical commodities.


% As per \Cref{thm:optimalmech}, in the event that the seller possesses the ability to customize data, she can achieve the first-best revenue and eliminate all of the buyer's surplus. 


\subsection{Selling Existing Data Records with Limited Customization
%Suboptimal Mechanism When the Seller Produces First
}\label{sec:subopt}
% {should we draw the timing lines?}
% Now, we focus on the situation in that the seller has no customization ability. Consider the model in \Cref{BLR}. For sellers without customized products, they can only produce items before buyers announce their types. Therefore, the timeline is that the seller produces $n$ data points first in what she likes directions. Then, the buyer reports his type, i.e. the direction he cares about. Recall that we don't make any assumptions about the truthfulness of the buyer. Then, the seller may process the data she has so as to achieve higher revenue and then gives the buyer dataset $\cD(\hat x)$ and charges $t(\hat x)$.

We now focus on the case where the seller has no perfect ability to customize her products. Consider again the model depicted in \Cref{BLR}. In cases where the seller cannot offer customized products, they are only able to produce items prior to the buyer declaring his preference. {However, the seller can transfer her owned dataset and that's why we call it ``limited''. After that, she will give the processed dataset to the buyer in order to recognize whether his feature is associated with a high willingness to pay and get it. By dealing with data rather than just giving out what she has, the seller may motivate the buyer to report truthfully. The trade-off becomes the loss of not giving out the whole dataset and the gain from price discrimination and we will prove in the following that it's impossible to achieve the first-best revenue in general cases under limited customization. }Thus, the timeline for this scenario involves the seller first producing $n$ data points in the directions she {is able to}. Following this, the buyer will report his preference, which is the direction that he {might be} interested in. It is important to note that we are not making any assumptions about the truthfulness of the buyer. Subsequently, the seller may process the data she has acquired so as to maximize her revenue. Then, the buyer will receive the dataset 
$\cD[\hat x]$ and be charged $t(\hat x)$. We visualize the timeline in \Cref{fig:limited}.

\begin{figure}[!htbp]
    \centering
    \includegraphics[width=\textwidth]{sections/imperfect.jpg}
    \caption{Timing line for limited data customization. {The first step is that the seller announces the upcoming mechanism and shows the dataset possibly only the design matrix she owns. In the second step, the buyer with private type $x$ decides to report that his type is $\hat x$. Based on the report $\hat x$, the seller will process the original dataset and finally gives out $\cD[\hat x]$ and charges $t(\hat x)$.}}
    \label{fig:limited}
\end{figure}

{Recall that in \Cref{example:drug}, Pfizer asks Hospital B for data to examine the efficacy of its new drug. The second approach that Hospital B provides Pfizer with the results of previous lung cancer patients who have used other drugs is a kind of limited data customization. The hospital can only give Pfizer data based on previous observations but not produce new data after observing Pfizer's requirements. Nevertheless, these preexisting data are still useful to Pfizer as it can use methods like synthetic control~\citep{bonander2017compared,abadie2021using} to learn the effect of the new drug. It reflects widespread applications of limited data customization models in the real world.}

Let us now formally examine the data that the seller has. The seller produces $n$ data points 
$\{(x_i,y_i)\}_{i=1}^n$. Here, 
$y_i=x_i^T\beta+\epsilon$, where $\epsilon$ follows a normal distribution with mean 0 and variance 
$\sigma(x_i)^2$. For simplicity, let 
$\cD\in\RR_{n\times d}$ denote the design matrix {of the whole dataset with a little abuse of notations} and $
Y$ the corresponding responses. We use 
$\Sigma(\cD)$ to represent the noise covariance matrix, i.e.
$\Sigma(\cD) = \diag\{\sigma(x_1)^2,...,\sigma(x_n)^2\}$.

% We formally show the data the seller has. She decides to produce $n$ data points denoted by $\{(x_i,y_i)\}_{i=1}^n$ and $y_i=x_i^T\beta+\epsilon$ where $\epsilon\sim \cN(0,\sigma(x_i)^2)$. For simplicity, we use $\cD\in\RR_{n\times d}$ and $Y$ to denote the design matrix and corresponding labels, respectively. Also, we use $\Sigma(\cD)$ to denote the noise covariance matrix $\diag\{\sigma(x_1)^2,...,\sigma(x_n)^2\}$. 

% Under this kind of information flow, the buyer won't suffer as much unfairness as the situation in \Cref{sec:optimal}. It means that customization may result in a bad effect on society and raise the question of how to constrain market power in the data market. However, on the other hand, the buyer's surplus will be upper bounded by a constant as follows and it does mean that in such a monopoly market, buyers are hard to access a high surplus. 

In this particular type of information flow, the buyer will not experience as much unfairness as the one in the situation described in \Cref{sec:optimal}. This implies that offering customization options may have negative consequences for society, and raises questions about how to regulate market power in the data market. However, it is important to note that the buyer's surplus will be bounded from above by a constant {unrelated to the buyer's type $x$}, which means that in a monopolized market, buyers will likely find it difficult to attain high surplus.

% Now, let's state our main results in the following theorems. For now, we will show the impossibility to achieve the first-best revenue for the seller. Like \Cref{sec:optimal}, we only need to consider mechanisms satisfying IC and IR constraints.

We now present our main results in the form of the following theorems. We first demonstrate the impossibility of achieving first-best revenue for the seller. Similar to \Cref{sec:optimal}, we only consider mechanisms that satisfy both IC and IR constraints, {that is, 
\begin{align*}
    &\textrm{IR}  &\IG(x, x) &\geq t(x)\textrm{ for all }x,\\
    \label{eq:defn_ic}
    &\textrm{IC}  &\IG(x, x) - t({x}) &\geq\IG(x, \hat x) - t(\hat x) \textrm{ for all }x, \hat{x}.
\end{align*}
}{As we discussed before, if it's impossible to achieve the first-best revenue in this subclass of mechanisms, there won't exist a mechanism achieving the first-best revenue among all unconstrained mechanisms.}
\begin{theorem}\label{thm:imposs}
When the type space is continuous, there is no mechanism that achieves the first-best revenue for all prior distributions of the buyer's type $x$.
\end{theorem}

{Despite the nuanced distinction between perfect data customization and limited data customization, \Cref{thm:imposs} together with \Cref{thm:optimalmech}, highlights essential differences of the fairness in the data pricing market.}

% Since we already have an upper-bound, first-price revenue, for any mechanism, we want to study the allocation of surplus between the seller and the buyer and the corresponding fairness in this data price. We will show in the following that the expectation of the buyer's surplus is less than a constant with respect to pre-produced $\cD$. We have the following theorem to show the imbalance of the market.

Given that we already have an upper bound for any mechanism, that is, the first-price revenue, we are interested in studying the division of the surplus between the seller and the buyer. In the following, we shall demonstrate that the expected surplus of the buyer with respect to the pre-produced $\cD$ is less than a constant. We formalize the result as follows.

\begin{theorem}\label{thm:surplusucb}
    For any pre-produced dataset $\cD$, the expectation of buyer's surplus is no larger than $\log(\kappa((\sqrt{\Sigma(\cD)})^{-1}\cD))$, where $\kappa((\sqrt{\Sigma(\cD)})^{-1}\cD)$ is the square root of the ratio between the largest and the smallest singular values of $\cD^T\Sigma(\cD)^{-1}\cD$.
\end{theorem}

% \Cref{thm:surplusucb} shows that though the seller cannot achieve the first-best revenue, the buyer's surplus is also upper-bounded by a constant only relative to pre-produced $\cD$ instead of his personal own type $x$. For different personal types, the buyer may have different consumer surplus, while the union upper bound holds for all types $x$.


As demonstrated by \Cref{thm:surplusucb}, even though the seller cannot achieve the first-best revenue, the buyer's surplus is also upper bounded by a constant relative only to the pre-produced 
$\cD$, rather than his personal type 
$x$. It is important to note that the buyer may have varying consumer surpluses for different personal types, while the union of upper bounds holds for all types 
$x$.{The proof of} \Cref{thm:surplusucb} leads to the following corollary about the seller that she can achieve within an additive factor of $\log(\kappa)$ of the first-best revenue.

\begin{corollary}\label{coroll:surplus}
    For any pre-produced dataset $\cD$, there exists a mechanism in which the expectation of the seller's revenue is at most $\log(\kappa((\sqrt{\Sigma(\cD)})^{-1}\cD))$ less than the first-best revenue.
\end{corollary}

{Together with \Cref{thm:surplusucb}, \Cref{coroll:surplus} gives an illustration of the ability of price discrimination under limited customization. Unlike perfect customization, the seller cannot achieve the first-best revenue in all cases. In other words, the worst-case distance between optimal revenue and the first-best revenue is strictly positive which infers that limited customization limits the level of market unfairness. However, it also shows that though the buyer could get a non-zero consumer surplus, it's indeed little and he still suffers inequality against the seller.}

The following results further show that for certain $\cD$, the seller can achieve the first-best revenue, highlighting the potential unfairness in the data market even under limited customization.

\begin{corollary}\label{thm:isotropic}
            When the seller has isotropic data, i.e. all singular values of $\cD^T\Sigma(\cD)^{-1}\cD$ are the same, there exists a mechanism that satisfies both IC and IR, and achieves the first-best revenue.
\end{corollary}

{At the same time, if the private types of the buyer which are public knowledge have certain structures, it's also possible for the seller to achieve the first-best revenue. As a kind of example, we introduce a new information structure called multi-armed bandits setting which also leads to the first-best revenue for the seller.
\begin{definition}
    We call a setting having a form of multi-armed bandits if every type vector $x$ is a member of the standard basis of a $d$-dimensional Euclidean space $\RR^{d}$. In other words, only one component of $x$ is one and the others are all zeros. 
\end{definition}
It is closely related to multi-armed bandits, the famous machine learning model. In multi-armed bandits, observations of rewards of one arm contain no information about rewards of other arms. In the data pricing, the multi-armed bandits setting means that data points associated with type $x$ involve no information about other types. Using a geometric perspective, it illustrates that the information corresponding to different types is orthogonal. Now, we have a corollary in which the seller can obtain the first-best revenue.}
\begin{corollary}\label{thm:mab}
            In the multi-armed bandits (MAB) setting, there exists a mechanism that satisfies both IC and IR, and achieves the first-best revenue.
\end{corollary}



{Together with \Cref{thm:surplusucb}, \Cref{thm:isotropic,thm:mab} show that the quantity of the consumer surplus not only depends on the concrete properties of the dataset $\cD$, but probably related information contained in the structure of the buyer's private types as well.}

% For the general theorem \Cref{thm:surplusucb}, since the different directions of data have different values to the buyer, the seller has incentives to motivate the buyer with a higher willingness to pay to report his type truthfully. In order to design a truthful mechanism, the seller needs to give up some charge in certain cases to achieve the highest expectation of revenue.  
In light of the universal \Cref{thm:surplusucb}, insofar as the diverse directions of data hold distinct values for the buyer, the seller harbors a motivation to induce the buyer, possessing a greater willingness to pay, to disclose his authentic type. To devise a truthful mechanism, the seller must relinquish some charge in specific instances to attain the maximum expected revenue.


% However, in \Cref{thm:isotropic}, every direction is isotropic and leads to the same value for the buyer. Therefore, it reveals the buyer's willingness to pay which is important for the seller to do price discrimination. It sheds light on the mechanism design problem in the data market that what's important to the seller is not the buyer's personal type but the willingness to pay. 


Notwithstanding, as per \Cref{thm:isotropic}, if each direction is isotropic, then it will confer equal value to the buyer. Hence, it discloses the buyer's willingness to pay, which is pivotal for the seller to implement price discrimination. It illuminates the {crucial point} of mechanism design in the data market, where the seller's focus is not on the buyers' individual type, but rather on their willingness to pay.

% Moreover, \Cref{thm:mab} shows the significance of information leakage. In the MAB setting, data of different directions gives no benefit to the buyer. As a result, the buyer has no intention to misreport and there is a natural price discrimination scenario.

\Cref{thm:mab} highlights the role of information leakage. In the context of multi-armed bandits, data from other arms provides no information then no benefit to the buyer, dissuading the buyer from untruthful reports, creating a natural case of price discrimination.

% {need more time to write the proof}








==> sections/opt.tex <==


\section{The Optimal Mechanism under Perfect Data Customization}\label{sec:optimal}
% We first consider the following information flow which represents customization. Considering the model in \Cref{BLR}, the buyer has private type $x$ and reports $\hat x$ to the seller. The seller can help the buyer to gain customized data $\hat y=\langle \hat x, \beta\rangle+\epsilon$ where $\epsilon\sim\cN(0,\sigma(\hat x)^2)$. For simplicity, we assume the quantity of data is known and denoted by $n$. With unknown $n$, the seller will use the mechanism below and her own cost function to derive optimal $n$. Readers can learn more about cost function in \citet{herzog2010theory}. Since the seller hopes to achieve price discrimination, she would like to add some man-made noise $\epsilon'$. We assume that $\epsilon'\sim \cN(0,\delta(\hat x)^2)$. Then, the seller charges the buyer $t(\hat x)$ which contains $n$ implicitly.

% With the definition of $\IG(\cdot,\cdot)$ in \Cref{eq:def-val-ig}, we have the following lemma about the value of data. We assume that the prior distribution is $\cN(0,I_d)$\footnote{We don't use the characteristic that $\beta$ is finite-dimensional and it can be extended to reproducing kernel Hilbert space directly.} W.L.O.G. If $\Var(\beta_q)$ is not full-rank, it means that some directions are deterministic and we can simply wipe off them. For general priori $\cN(\beta_0,\Sigma_0)$, we can subtract every $y$ by $x^T\beta_0$ to reduce to the situation of $\cN(0,\Sigma_0)$. Then, we can replace $(x,\beta)$ by $(\sqrt{\Sigma_0}x,(\sqrt{\Sigma_0})^{-1}\beta)$ and it reduces to our assumption.

We begin with the case where the seller can customize her data perfectly. {Recall that we use ``customize'' to represent the seller will distribute different data after observing different reports of the buyer's type. ``Perfect'' here means that the seller can generate data after observing the report like in \Cref{fig:perfect} while we will use ``limited'' to represent the situation in which the seller generates data before receiving reports. We note that customization scenario often occurs between pharmaceutical companies and hospitals. Pharmaceutical companies hope that hospitals can help them evaluate the effectiveness of newly developed drugs. Therefore, pharmaceutical companies will pay for experiments conducted in hospitals. Although hospitals may not have the capability to produce drugs, they can provide observational data on the efficacy of drugs for pharmaceutical companies. We first adopt the following example to illustrate scenarios of perfect data customization. 
\begin{example}[Drug efficacy assessment]\label{example:drug}
    Pfizer has developed a new drug for the treatment of lung cancer and is seeking to conduct drug testing at Hospital B. Hospital B provided Pfizer with the following two options. 
    \begin{itemize}
        \item Hospital B directly conducts experiments on patients using the drug and returns clinical outcomes to Pfizer.
        \item Hospital B provides Pfizer with the results of previous lung cancer patients who have used other drugs.
    \end{itemize}
    Both options are beneficial for Pfizer to assess the effectiveness of the new drug and present different mechanism design problems for the study protocols.
\end{example}
In \Cref{example:drug}, the first option that the hospital uses drugs provided by Pfizer on patients directly is a kind of scenario of perfect data customization in the real world. In abstract terms, no matter what feature vector the buyer is interested in, the seller has the capability to generate precisely the data that the buyer desires.
}

In reference to the model displayed in \Cref{BLR}, the buyer is equipped with some {fixed} type vector $x$ in favor of related data-generating process and sends $\hat x$ to the seller, {akin to settings of mechanism design literature~\citep{myerson1979incentive,bull2007hard,borgers2015introduction}}. {$x$ and $\hat x$ might be different as the buyer pretends to ask for data corresponding to the direction of $\hat x$ in order to reduce the payment. }In the perfect customization case, the seller can directly, and potentially repeatedly, observe the response which corresponds to $\hat{x}$, namely $\hat y=\langle \hat x, \beta\rangle+\epsilon$, where $\epsilon\sim\cN(0,\sigma(\hat x)^2)$. For simplicity, we assume that the seller receives
$n$ measurements of $\hat{y}$, jointly independent when conditioned on $\hat{x}$ and $\beta$. {The size of the dataset, i.e. $n$, might depend on the cost of generating data and the budget constraints faced by the buyer which is exogenous and independent of our mechanism design. When $n$ is unknown, the seller will employ the following proposed mechanism in \Cref{algo:opt} concurrently with her personal cost function to derive the optimal $n$. We refer readers interested in further information on the cost function to \citet{herzog2010theory}. For the convenience of understanding, we assume $n$ is fixed from now on.}
% When the seller is $n$ is unknown, the seller will employ the following mechanism in conjunction with her personal cost function to derive the optimal 
% $n$. We refer readers interested in further information on the cost function to \citet{herzog2010theory}. 
In order to increase revenue, the seller may inject into the responses some artificial noise denoted by $\epsilon'$, where 
$\epsilon'\sim \cN(0,\delta(\hat x)^2)$. {The idea behind these artificial noises is that the seller hopes they can help distinguish buyers with a better willingness to pay. By injecting noise, it might punish buyers who misreport their own types and motivate a truthful mechanism. Then, they can utilize price discrimination to obtain higher expected revenue.} The seller then charges the buyer 
$t(\hat x)$, which may depend on 
$n$, {the number of data point in the dataset}. The exact timing line is provided in \Cref{fig:perfect}.

\begin{figure}[!htbp]
    \centering
    \includegraphics[width=\textwidth]{sections/perfect.jpg}
    \caption{Timing line for perfect data customization. {The first step is to announce the mechanism to be used. Then, the buyer who is equipped with type $x$ gives a report $\hat x$ to the seller. The seller will base on $\hat x$ to produce a dataset we call $\cD[\hat x]$ and give it to the buyer. Finally, the buyer will give the seller a preset fee $t(\hat x)$.}}
    \label{fig:perfect}
\end{figure}

We assume without loss of generality {there is a common knowledge} that the prior distribution \hfr{over $\beta$} is 
$\cN(0,I_d)$\footnote{We do not use the fact that 
$\beta$ is finite-dimensional and our results can be directly extended to reproducing kernel Hilbert space.}{, which is standard in information economy literature~\citep{frankel2019quantifying,hartline2010bayesian,maschler2020game}.} If 
$\Var(\beta_q)$, {the variance matrix of the prior parameter,}
is not full-rank, this implies that certain directions are deterministic and can be disregarded. For a general priori 
$\cN(\beta_q,\Sigma_0)$, we can subtract every 
$y$ by 
$x^T\beta_q$ to simplify the situation to 
$\cN(0,\Sigma_0)$. Subsequently, we can replace 
$(x,\beta)$ by 
$(\sqrt{\Sigma_0}x,(\sqrt{\Sigma_0})^{-1}\beta)$ and it will reduce to our initial assumption.

Concerning the definition of $\IG(\cdot;\cdot,\cdot)$ in \Cref{eq:value-linear-dpp}, we can establish a lemma exhibiting the
concrete instrumental value of data in detail.
\begin{lemma}\label{lem:concrete_value}
    If the seller gives the buyer $n$ data points, it holds that the instrumental value of data
for the buyer is
\[
\IG(x, \widehat{x}):=\IG( \cD[\widehat{x}];\cN(0,I_d),x)=\frac{1}{2} \log \left(x^T x\right)-\frac{1}{2} \log \left(x^T\left(I+\frac{n \widehat{x} \widehat{x}^T}{\sigma(\widehat{x})^2+\delta(\widehat{x})^2}\right)^{-1} x\right).
\]
\end{lemma}

% With revelation principle \citep{gibbard1973manipulation,holmstrom1978incentives,myerson1979incentive}, we only consider the incentive-compatibility (IC) mechanism. Since the buyer is assumed rational, the mechanism should satisfy individual rationality (IR) constraints. Therefore, we formally state the following constraints that the mechanism should obey.
By revelation principle \citep{gibbard1973manipulation,holmstrom1978incentives,myerson1979incentive}, {we know that any social choice function implemented by an arbitrary mechanism can be implemented by an incentive-compatible-direct-mechanism with the same equilibrium outcome.} Therefore, we focus on mechanisms that satisfy incentive-compatibility (IC) constraint and {at least one optimal mechanism belongs to this subclass. In the context of our model, incentive-compatibility constraint means that the buyer has the motivation to report his own private type truthfully considering the allocation rule $\cD[\cdot]$ and payment rule $t(\cdot)$.} To ensure the buyer is motivated to purchase data, we further impose individual rationality (IR) constraints. {It means that a rational buyer only participates in a transaction when his expected revenue is no less than zero. }Formally, the IC and IR constraints for a mechanism $(\cD[\cdot], t(\cdot))$ are
\begin{align*}
    \label{eq:defn_ir}
    &\textrm{IR}  &\IG(x, x) &\geq t(x)\textrm{ for all }x,\\
    % \label{eq:defn_ic}
    &\textrm{IC}  &\IG(x, x) - t({x}) &\geq \IG(x, \hat x) - t(\hat x)\textrm{ for all }x, \hat{x} .
\end{align*}
{In other words, IC constraint means that truthful reporting is a dominant strategy for the buyer and he has no incentive to report a wrong type as there are no benefits by doing so. IR constraint gives the buyer a reason to join the market and motivates the transaction as his expected utility is non-negative.}

We further make an assumption on the data-generating model. {We assume the variance is scaled to the norm of the feature as follows.}
\begin{assumption}\label{assumption:scale}
The noise's variance scales with the length of $x$, i.e. $\sigma(x)=\sigma(\frac{x}{\|x\|})\|x\|.$
\end{assumption}

% Assumption \ref{assumption:scale} is a quite normal assumption in physics literature and biomedicine literature \citep{linnet1990estimation,kumar1994proportional,bland1996measurement} as the measurement error is often proportional to the quantitative of the variable. Also, we constrain the additive noise $\epsilon'$ also have a proportional variance that 
% \[
% \delta(x)=\delta(\frac{x}{\|x\|})\|x\|,
% \]which may reduce the seller's revenue. However, we will show as follows that such a family of mechanisms can already achieve the first-best revenue so the mechanism we propose is indeed the optimal mechanism.


Assumption \ref{assumption:scale} is commonplace in the literature of physics and biomedicine \citep{linnet1990estimation,kumar1994proportional,bland1996measurement,wang2006proportional}, as the measurement error is frequently proportional to the ``size'' of the variable being measured and here ``size'' is quantified by $\| \cdot \|$. Similarly, we stipulate that the additional noise 
$\epsilon'$ also has a proportional variance defined by $\delta(x)=\delta(\frac{x}{\|x\|})\|x\|$, which may decrease the revenue obtained by the seller. Nevertheless, we will demonstrate that this family of mechanisms is capable of achieving the first-best revenue and, by extension, optimality.

% With Assumption \ref{assumption:scale} in hand, it's obvious that we only can only consider the direction of type rather than the length. We can replace $x$ and $\hat x$ by $\frac{x}{\|x\|}$ and $\frac{\hat x}{\|\hat x\|}$ and it holds that
% \[
% \IG( x,\hat x)=\IG(\frac{x}{\| x\|},\frac{\hat x}{\|\hat x\|}).
% \]
% From now on, we only consider types belonging to $\{x:\|x\|=1\}$.
Given Assumption \ref{assumption:scale}, it is evident that we could solely consider the direction of the type, rather than its length. This can be achieved by substituting 
$x$ and $\hat x$
  with 
$\frac{x}{\|x\|}$ and $\frac{\hat x}{\|\hat x\|}$, respectively. We then have
\[
\IG( x,\hat x)=\IG(\frac{x}{\| x\|},\frac{\hat x}{\|\hat x\|}).
\]
We thus restrict our attention to types with a unit norm, i.e. 
$\cS^{d-1}=\{x:\|x\|=1\}$, {which is equivalent to considering a general space in $\RR^{d-1}$}. Inspired by the method in \citet{myerson1981optimal}, we have the following lemma when $x$ has multiple dimensions.
\begin{lemma}\label{lem:paymentgrad}
    For any payment rule satisfying the IC constraint, it holds that
\[
\nabla t(x)=\nabla_y \IG(x,y)\given_{y=x}.
\]
Therefore, it leads to the following form of payment rule that
\[
t(x)=\int_{x_0}^x \nabla_y \IG(x,y)\given_{y=x}\cdot dx+t(x_0)=\frac{1}{2}\log(\frac{\sigma(x)^2+\delta(x)^2+n}{\sigma(x)^2+\delta(x)^2})+C,
\]
and it's independent of the selection of $x_0$ and the path of integration.
\end{lemma}
{Compared with the well-known results of single-dimension in \citet{myerson1981optimal}, there are two main differences considering a multi-dimensional type. First of all, we need to generalize the derivation of a one-dimensional function to the gradient computation in the case of higher dimensions. Second, when calculating the payment rule $t(\cdot)$, the integral result is required to be independent of the initial starting point and the integral path we choose. In our situation, it means that no matter what $x_0$ and the path from it to the final $x$ we choose, the result of the integral should be the same. These conditions constrain the application scenarios of the extended method for multi-dimensional mechanism design as we only need monotonicity for the single-dimensional situation. Nevertheless, the proof will elaborate that our definition of instrumental value satisfies all these conditional endogenously, highlighting the importance of our framework of instrumental value and suggesting its broad range of applications.}

Therefore, for any $\delta(x)$, we have the corresponding optimization problem for optimal mechanism, that is
\begin{equation*}\label{optimization_problem}
      \max_{C,\delta(\cdot)} \EE_x t(x)=\EE_x [C+\frac{1}{2}\log(\frac{\sigma(x)^2+\delta(x)^2+n}{\sigma(x)^2+\delta(x)^2})]\ind({\rm IR\ holds}),
\end{equation*}
where $$\ind({\rm IR\ holds})=
  \ind(C+\frac{1}{2}\log(\frac{\sigma(x)^2+\delta(x)^2+n}{\sigma(x)^2+\delta(x)^2})+\frac{1}{2}\log(x^T(I+\frac{nxx^T}{\sigma(x)^2+\delta(x)^2})^{-1}x)\le 0).$$  

{Though information gain is a widely used metric, our analysis method can be extended to a wider family of instrumental values as long as keeping the concavity property as what $\log(\cdot)$ does. We add the following remark to show how to generalize our results.} 
\begin{remark}
The method can be easily extended to any $\IG(\cdot,\cdot)$ function following the form
\[
\IG(x,\hat x)=f(\frac{x^Tx}{x^T(I+\frac{\hat x\hat x^T}{(\sigma(\hat x)^2+\delta(\hat x)^2)/n})^{-1}x}),
\]
where $f(\cdot)$ is a concave function, and the results remain valid when $t(x)$ is of the form
\[
t(x)=C+f(\frac{\sigma(x)^2+\delta(x)^2+n}{\sigma(x)^2+\delta(x)^2}).
\]
\end{remark}

We now state our main result. {It shows that when the seller is embedded with the ability of perfect customization, she can obtain the first-best revenue and leave zero consumer surplus to the buyer. It reflects the price discrimination scenario in the data market and shows corresponding unfairness which is quite different than the situation in other markets.}
\begin{theorem}\label{thm:optimalmech}    {There exists a mechanism satisfying both IC and IR constraints} that for any $\sigma(\cdot)$ and prior distribution on the type $x$, the seller can achieve the first-best revenue and first-degree price discrimination, where the corresponding payment rule is 
    \[
    t(x)=\frac{1}{2}\log(\frac{\sigma(x)^2+n}{\sigma(x)^2}).
    \]
\end{theorem}

% We formalize \Cref{thm:optimalmech} in \Cref{algo:opt}. \Cref{algo:opt} shows in detail that when the seller has customization ability, there's no need for her to add additional noise besides endogenous ones. She can abstract the buyer's willingness to pay exactly since data in different directions may impair the buyer's valuation heavily. Therefore, for sellers with perfect data customization ability, it's achievable for them to achieve the first-best revenue with unfairness to buyers and society. 
We present an optimal mechanism constructed by \Cref{thm:optimalmech} in \Cref{algo:opt}. As demonstrated in \Cref{algo:opt}, when the seller can perfectly customize data, it is unnecessary for her to inject any additional noise. She can fully extract the buyer's willingness to pay since the value of data significantly degrades once the buyer alters the direction of the reported type. Consequently, for sellers with perfect data customization ability, it is feasible for them to achieve the first-best revenue at the expense of the buyers, {where the sellers seize all the surplus and none are left to the buyers}. Moreover, there is no deadweight loss (see \citet{hausman1981exact} for detailed concepts) since she is selling as much information as possible, without injecting any artificial noise, and the buyer has no further willingness to pay. The result stands in {distinct} contrast to the corresponding market forms for physical commodities.

% \begin{algorithm}[thbp]
% \renewcommand{\algorithmicrequire}{\textbf{Input:}}
% \renewcommand{\algorithmicensure}{\textbf{Output:}}
%     \begin{algorithmic}
%     \REQUIRE{buyer's report $\hat x$}
%     \STATE Set $\delta(\cdot)\equiv 0$ for the distribution of added noise $\cN(0,\delta(\cdot)^2)$
%     \STATE The seller generates $n$ data \hf{Is $n$ a design parameter, or a given fixed value in advance?} points following $\hat y_i=\hat x^T\beta+\epsilon_i+\epsilon'_i$ where $\epsilon'_i\overset{\text{i.i.d.}}{\sim}\cN(0,\delta(\hat x)^2)$
%     \ENSURE {
%          $\cD[\hat{x}] = \{(\hat x ,\hat y_i)\}_{i=1}^n$ and $t(\hat x)=\frac{1}{2}\log(\frac{\sigma(\hat x)^2+n}{\sigma(\hat x)^2})$
% }\label{algo:allocation}\label{algo:payment}
%     % Set $t(\hat{x}) = \IG(\hat x, \cD(\hat{x})) =\frac{1}{2}\log(\hat x^T\hat x)-\frac{1}{2}\log(\hat x^T(I+\sellX^Tb(\hat x)b(\hat x)^T\sellX)^{-1}\hat x)$\;
%     \caption{Pseudocode for the Optimal Mechanism}
%     \label{algo:opt}
%     \end{algorithmic}
% \end{algorithm}

% \begin{algorithm}[t]    
% 	\SetAlgoNoLine
% 	\KwIn{buyer's report $\hat x$}
% 	Set $\delta(\cdot)\equiv 0$ for the distribution of added noise $\cN(0,\delta(\cdot)^2)$\;
%  The seller generates $n$ data 
%  % \hf{Is $n$ a design parameter, or a given fixed value in advance?}
%  points following $\hat y_i=\hat x^T\beta+\epsilon_i+\epsilon'_i$ where $\epsilon'_i\overset{\text{i.i.d.}}{\sim}\cN(0,\delta(\hat x)^2)$\;
% 	\KwOut{$\cD[\hat{x}] = \{(\hat x ,\hat y_i)\}_{i=1}^n$ and $t(\hat x)=\frac{1}{2}\log(\frac{\sigma(\hat x)^2+n}{\sigma(\hat x)^2})$}\label{algo:allocation}\label{algo:payment}
% 	\caption{Pseudocode for the Optimal Mechanism}
%         \label{algo:opt}
% \end{algorithm}

\begin{algorithm}[htbp]
   \caption{Pseudocode for the Optimal Mechanism}
        \label{algo:opt}
\begin{algorithmic}
   \STATE {\bfseries Input:} buyer's report $\hat x$
   \STATE Set $\delta(\cdot)\equiv 0$ for the distribution of added noise $\cN(0,\delta(\cdot)^2)$;
   \STATE  The seller generates $n$ data 
 % \hf{Is $n$ a design parameter, or a given fixed value in advance?}
 points following $\hat y_i=\hat x^T\beta+\epsilon_i+\epsilon'_i$ where $\epsilon'_i\overset{\text{i.i.d.}}{\sim}\cN(0,\delta(\hat x)^2)$;
    \STATE {\bfseries Output:} $\cD[\hat{x}] = \{(\hat x ,\hat y_i)\}_{i=1}^n$ and $t(\hat x)=\frac{1}{2}\log(\frac{\sigma(\hat x)^2+n}{\sigma(\hat x)^2})$\label{algo:allocation}\label{algo:payment}
\end{algorithmic}
\end{algorithm}


% \Cref{thm:optimalmech} shows that when the seller has customization ability, she can achieve first price revenue and subtracts all buyer's surplus. At the same time, there's no deadweight loss (see \citet{hausman1981exact} for detailed concepts) that she sells as much information as she can and the buyer has no more willingness to pay. So, under this information flow, there is a market with unfairness that the buyer enjoys no surplus and it shows large differences with corresponding market forms for physical commodities.


% As per \Cref{thm:optimalmech}, in the event that the seller possesses the ability to customize data, she can achieve the first-best revenue and eliminate all of the buyer's surplus. 









==> sections/subopt.tex <==
\section{Mechanisms under Limited Data Customization 
%Suboptimal Mechanism When the Seller Produces First
}\label{sec:subopt}
% {should we draw the timing lines?}
% Now, we focus on the situation in that the seller has no customization ability. Consider the model in \Cref{BLR}. For sellers without customized products, they can only produce items before buyers announce their types. Therefore, the timeline is that the seller produces $n$ data points first in what she likes directions. Then, the buyer reports his type, i.e. the direction he cares about. Recall that we don't make any assumptions about the truthfulness of the buyer. Then, the seller may process the data she has so as to achieve higher revenue and then gives the buyer dataset $\cD(\hat x)$ and charges $t(\hat x)$.

We now focus on the case where the seller has no perfect ability to customize her products. Consider again the model depicted in \Cref{BLR}. In cases where the seller cannot offer customized products, they are only able to produce items prior to the buyer declaring his preference. {However, the seller can transfer her owned dataset and that's why we call it ``limited''. After that, she will give the processed dataset to the buyer in order to recognize whether his feature is associated with a high willingness to pay and get it. By dealing with data rather than just giving out what she has, the seller may motivate the buyer to report truthfully. The trade-off becomes the loss of not giving out the whole dataset and the gain from price discrimination and we will prove in the following that it's impossible to achieve the first-best revenue in general cases under limited customization. }Thus, the timeline for this scenario involves the seller first producing $n$ data points in the directions she {is able to}. Following this, the buyer will report his preference, which is the direction that he {might be} interested in. It is important to note that we are not making any assumptions about the truthfulness of the buyer. Subsequently, the seller may process the data she has acquired so as to maximize her revenue. Then, the buyer will receive the dataset 
$\cD[\hat x]$ and be charged $t(\hat x)$. We visualize the timeline in \Cref{fig:limited}.

\begin{figure}[!htbp]
    \centering
    \includegraphics[width=\textwidth]{sections/imperfect.jpg}
    \caption{Timing line for limited data customization. {The first step is that the seller announces the upcoming mechanism and shows the dataset possibly only the design matrix she owns. In the second step, the buyer with private type $x$ decides to report that his type is $\hat x$. Based on the report $\hat x$, the seller will process the original dataset and finally gives out $\cD[\hat x]$ and charges $t(\hat x)$.}}
    \label{fig:limited}
\end{figure}

{Recall that in \Cref{example:drug}, Pfizer asks Hospital B for data to examine the efficacy of its new drug. The second approach that Hospital B provides Pfizer with the results of previous lung cancer patients who have used other drugs is a kind of limited data customization. The hospital can only give Pfizer data based on previous observations but not produce new data after observing Pfizer's requirements. Nevertheless, these preexisting data are still useful to Pfizer as it can use methods like synthetic control~\citep{bonander2017compared,abadie2021using} to learn the effect of the new drug. It reflects widespread applications of limited data customization models in the real world.}

Let us now formally examine the data that the seller has. The seller produces $n$ data points 
$\{(x_i,y_i)\}_{i=1}^n$. Here, 
$y_i=x_i^T\beta+\epsilon$, where $\epsilon$ follows a normal distribution with mean 0 and variance 
$\sigma(x_i)^2$. For simplicity, let 
$\cD\in\RR_{n\times d}$ denote the design matrix {of the whole dataset with a little abuse of notations} and $
Y$ the corresponding responses. We use 
$\Sigma(\cD)$ to represent the noise covariance matrix, i.e.
$\Sigma(\cD) = \diag\{\sigma(x_1)^2,...,\sigma(x_n)^2\}$.

% We formally show the data the seller has. She decides to produce $n$ data points denoted by $\{(x_i,y_i)\}_{i=1}^n$ and $y_i=x_i^T\beta+\epsilon$ where $\epsilon\sim \cN(0,\sigma(x_i)^2)$. For simplicity, we use $\cD\in\RR_{n\times d}$ and $Y$ to denote the design matrix and corresponding labels, respectively. Also, we use $\Sigma(\cD)$ to denote the noise covariance matrix $\diag\{\sigma(x_1)^2,...,\sigma(x_n)^2\}$. 

% Under this kind of information flow, the buyer won't suffer as much unfairness as the situation in \Cref{sec:optimal}. It means that customization may result in a bad effect on society and raise the question of how to constrain market power in the data market. However, on the other hand, the buyer's surplus will be upper bounded by a constant as follows and it does mean that in such a monopoly market, buyers are hard to access a high surplus. 

In this particular type of information flow, the buyer will not experience as much unfairness as the one in the situation described in \Cref{sec:optimal}. This implies that offering customization options may have negative consequences for society, and raises questions about how to regulate market power in the data market. However, it is important to note that the buyer's surplus will be bounded from above by a constant {unrelated to the buyer's type $x$}, which means that in a monopolized market, buyers will likely find it difficult to attain high surplus.

% Now, let's state our main results in the following theorems. For now, we will show the impossibility to achieve the first-best revenue for the seller. Like \Cref{sec:optimal}, we only need to consider mechanisms satisfying IC and IR constraints.

We now present our main results in the form of the following theorems. We first demonstrate the impossibility of achieving first-best revenue for the seller. Similar to \Cref{sec:optimal}, we only consider mechanisms that satisfy both IC and IR constraints, {that is, 
\begin{align*}
    &\textrm{IR}  &\IG(x, x) &\geq t(x)\textrm{ for all }x,\\
    \label{eq:defn_ic}
    &\textrm{IC}  &\IG(x, x) - t({x}) &\geq\IG(x, \hat x) - t(\hat x) \textrm{ for all }x, \hat{x}.
\end{align*}
}{As we discussed before, if it's impossible to achieve the first-best revenue in this subclass of mechanisms, there won't exist a mechanism achieving the first-best revenue among all unconstrained mechanisms.}
\begin{theorem}\label{thm:imposs}
When the type space is continuous, there is no mechanism that achieves the first-best revenue for all prior distributions of the buyer's type $x$.
\end{theorem}

{Despite the nuanced distinction between perfect data customization and limited data customization, \Cref{thm:imposs} together with \Cref{thm:optimalmech}, highlights essential differences of the fairness in the data pricing market.}

% Since we already have an upper-bound, first-price revenue, for any mechanism, we want to study the allocation of surplus between the seller and the buyer and the corresponding fairness in this data price. We will show in the following that the expectation of the buyer's surplus is less than a constant with respect to pre-produced $\cD$. We have the following theorem to show the imbalance of the market.

Given that we already have an upper bound for any mechanism, that is, the first-price revenue, we are interested in studying the division of the surplus between the seller and the buyer. In the following, we shall demonstrate that the expected surplus of the buyer with respect to the pre-produced $\cD$ is less than a constant. We formalize the result as follows.

\begin{theorem}\label{thm:surplusucb}
    For any pre-produced dataset $\cD$, the expectation of buyer's surplus is no larger than $\log(\kappa((\sqrt{\Sigma(\cD)})^{-1}\cD))$, where $\kappa((\sqrt{\Sigma(\cD)})^{-1}\cD)$ is the square root of the ratio between the largest and the smallest singular values of $\cD^T\Sigma(\cD)^{-1}\cD$.
\end{theorem}

% \Cref{thm:surplusucb} shows that though the seller cannot achieve the first-best revenue, the buyer's surplus is also upper-bounded by a constant only relative to pre-produced $\cD$ instead of his personal own type $x$. For different personal types, the buyer may have different consumer surplus, while the union upper bound holds for all types $x$.


As demonstrated by \Cref{thm:surplusucb}, even though the seller cannot achieve the first-best revenue, the buyer's surplus is also upper bounded by a constant relative only to the pre-produced 
$\cD$, rather than his personal type 
$x$. It is important to note that the buyer may have varying consumer surpluses for different personal types, while the union of upper bounds holds for all types 
$x$.{The proof of} \Cref{thm:surplusucb} leads to the following corollary about the seller that she can achieve within an additive factor of $\log(\kappa)$ of the first-best revenue.

\begin{corollary}\label{coroll:surplus}
    For any pre-produced dataset $\cD$, there exists a mechanism in which the expectation of the seller's revenue is at most $\log(\kappa((\sqrt{\Sigma(\cD)})^{-1}\cD))$ less than the first-best revenue.
\end{corollary}

{Together with \Cref{thm:surplusucb}, \Cref{coroll:surplus} gives an illustration of the ability of price discrimination under limited customization. Unlike perfect customization, the seller cannot achieve the first-best revenue in all cases. In other words, the worst-case distance between optimal revenue and the first-best revenue is strictly positive which infers that limited customization limits the level of market unfairness. However, it also shows that though the buyer could get a non-zero consumer surplus, it's indeed little and he still suffers inequality against the seller.}

The following results further show that for certain $\cD$, the seller can achieve the first-best revenue, highlighting the potential unfairness in the data market even under limited customization.

\begin{corollary}\label{thm:isotropic}
            When the seller has isotropic data, i.e. all singular values of $\cD^T\Sigma(\cD)^{-1}\cD$ are the same, there exists a mechanism that satisfies both IC and IR, and achieves the first-best revenue.
\end{corollary}

{At the same time, if the private types of the buyer which are public knowledge have certain structures, it's also possible for the seller to achieve the first-best revenue. As a kind of example, we introduce a new information structure called multi-armed bandits setting which also leads to the first-best revenue for the seller.
\begin{definition}
    We call a setting having a form of multi-armed bandits if every type vector $x$ is a member of the standard basis of a $d$-dimensional Euclidean space $\RR^{d}$. In other words, only one component of $x$ is one and the others are all zeros. 
\end{definition}
It is closely related to multi-armed bandits, the famous machine learning model. In multi-armed bandits, observations of rewards of one arm contain no information about rewards of other arms. In the data pricing, the multi-armed bandits setting means that data points associated with type $x$ involve no information about other types. Using a geometric perspective, it illustrates that the information corresponding to different types is orthogonal. Now, we have a corollary in which the seller can obtain the first-best revenue.}
\begin{corollary}\label{thm:mab}
            In the multi-armed bandits (MAB) setting, there exists a mechanism that satisfies both IC and IR, and achieves the first-best revenue.
\end{corollary}



{Together with \Cref{thm:surplusucb}, \Cref{thm:isotropic,thm:mab} show that the quantity of the consumer surplus not only depends on the concrete properties of the dataset $\cD$, but probably related information contained in the structure of the buyer's private types as well.}

% For the general theorem \Cref{thm:surplusucb}, since the different directions of data have different values to the buyer, the seller has incentives to motivate the buyer with a higher willingness to pay to report his type truthfully. In order to design a truthful mechanism, the seller needs to give up some charge in certain cases to achieve the highest expectation of revenue.  
In light of the universal \Cref{thm:surplusucb}, insofar as the diverse directions of data hold distinct values for the buyer, the seller harbors a motivation to induce the buyer, possessing a greater willingness to pay, to disclose his authentic type. To devise a truthful mechanism, the seller must relinquish some charge in specific instances to attain the maximum expected revenue.


% However, in \Cref{thm:isotropic}, every direction is isotropic and leads to the same value for the buyer. Therefore, it reveals the buyer's willingness to pay which is important for the seller to do price discrimination. It sheds light on the mechanism design problem in the data market that what's important to the seller is not the buyer's personal type but the willingness to pay. 


Notwithstanding, as per \Cref{thm:isotropic}, if each direction is isotropic, then it will confer equal value to the buyer. Hence, it discloses the buyer's willingness to pay, which is pivotal for the seller to implement price discrimination. It illuminates the {crucial point} of mechanism design in the data market, where the seller's focus is not on the buyers' individual type, but rather on their willingness to pay.

% Moreover, \Cref{thm:mab} shows the significance of information leakage. In the MAB setting, data of different directions gives no benefit to the buyer. As a result, the buyer has no intention to misreport and there is a natural price discrimination scenario.

\Cref{thm:mab} highlights the role of information leakage. In the context of multi-armed bandits, data from other arms provides no information then no benefit to the buyer, dissuading the buyer from untruthful reports, creating a natural case of price discrimination.

% {need more time to write the proof}

